Helping Hands: An Object-Aware Ego-Centric Video Recognition Model

We introduce an object-aware decoder for improving the performance of spatio-temporal representations on ego-centric videos. The key idea is to enhance object-awareness during training by tasking the model to predict hand positions, object positions, and the semantic label of the objects using paired captions when available. At inference time the model only requires RGB frames as inputs, and is able to track and ground objects (although it has not been trained explicitly for this). We demonstrate the performance of the object-aware representations learnt by our model, by: (i) evaluating it for strong transfer, i.e. through zero-shot testing, on a number of downstream video-text retrieval and classification benchmarks; and (ii) by using the representations learned as input for long-term video understanding tasks (e.g. Episodic Memory in Ego4D). In all cases the performance improves over the state of the art -- even compared to networks trained with far larger batch sizes. We also show that by using noisy image-level detection as pseudo-labels in training, the model learns to provide better bounding boxes using video consistency, as well as grounding the words in the associated text descriptions. Overall, we show that the model can act as a drop-in replacement for an ego-centric video model to improve performance through visual-text grounding.

==> tables/egomcq.tex <==
\begin{table}[]
\centering
\renewcommand*{\arraystretch}{1.1}

\resizebox{\linewidth}{!}{%
\begin{tabular}{ccc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & \multirow{2}{*}{\textbf{Object-aware}} & \multicolumn{2}{c}{\textbf{EgoMCQ}} \\
                                 &                                    &                                        & Inter-video      & Intra-video      \\ \hline
EgoVLP                           & TSF-B                              & N                                      & 90.6             & 57.2             \\
LaViLA                           & TSF-B                              & N                                      & 93.8             & 59.9             \\
LaViLA                           & TSF-L                              & N                                      & 94.5             & 63.1             \\ \hline
Ours                             & TSF-L                              & N                                      &                  &                  \\
Ours                             & TSF-L                              & Y                                      &                  &                  \\ \hline
\end{tabular}%
}
\vspace{1mm}
\caption{\textbf{Accuracy on EgoMCQ.}}
\label{tab:egomcq}
\end{table}

==> tables/ek_mir.tex <==
\begin{table}[]
\centering
\renewcommand*{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccc|ccc|ccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Backbone}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Object\\ aware\end{tabular}}} & \multicolumn{3}{c|}{\textbf{mAP}} & \multicolumn{3}{c}{nDCG} \\
                                 &                                    &                                                                                  & V-T       & T-V       & Avg       & V-T    & T-V    & Avg    \\ \hline
EgoVLP                           & TSF-B                              & N                                                                                & 26.0      & 20.6      & 23.3      & 28.8   & 27.0   & 27.9   \\
LaViLA                           & TSF-B                              & N                                                                                & 35.1      & 26.6      & 30.9      & 33.7   & 30.4   & 32.0   \\
LaViLA                           & TSF-L                              & N                                                                                & 40.0      & 32.2      & 36.1      & 36.1   & 33.2   & 34.6   \\ \hline
Ours                             & TSF-L                              & N                                                                                &           &           &           &        &        &        \\
Ours                             & TSF-L                              & N                                                                                &           &           &           &        &        &        \\
Ours                             & TSF-L                              & Y                                                                                &           &           &           &        &        &        \\ \hline
\end{tabular}%
}
\vspace{1mm}
\caption{\textbf{Zero-shot accuracy on EK-100 MIR}}
\label{tab:ek_mir}
\end{table}

==> tables/rebuttal_better_box.tex <==
\makeatletter         
\renewcommand\maketitle{
{}} % Note the extra }
\makeatother
\renewcommand*{\arraystretch}{0.6}
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\centering
\small
\begin{tabular}{cc|cccccc|cc|cccc}
\hline
\multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Detector \\ input res\end{tabular}}} & \multicolumn{6}{c|}{\textbf{EpicKitchens}}                                                    & \multicolumn{2}{c|}{\textbf{EGTEA}}           & \multicolumn{4}{c}{\textbf{EgoNLQ}}                         \\
                                 &                                                                                         & \multicolumn{3}{c}{mAP}                       & \multicolumn{3}{c|}{nDCG}                     & \multirow{2}{*}{Top1} & \multirow{2}{*}{Mean} & \multicolumn{2}{c}{mIOU@0.3} & \multicolumn{2}{c}{mIOU@0.5} \\
                                 &                                                                                         & V-T           & T-V           & Avg           & V-T           & T-V           & Avg           &                       &                       & R1            & R5           & R1            & R5           \\ \hline
\textbf{LaviLa}                  & -                                                                                       & 40.0          & 32.2          & 36.1          & 36.1          & 33.2          & 34.6          & 34.0                  & 40.1                  & 12.1          & 22.4         & 7.3           & 15.4         \\ \hline
\multirow{2}{*}{\textbf{Ours}}   & 256                                                                                     & 41.5          & 32.3          & 36.9          & 38.6          & 35.4          & 37.0          & 38.9                  & 44.3                  & 12.3          & 23.0         & 7.6           & \textbf{15.6}         \\
                                 & 640                                                                                     & \textbf{42.7} & \textbf{33.1} & \textbf{37.9} & \textbf{39.6} & \textbf{36.3} & \textbf{38.0} & \textbf{39.1}         & \textbf{46.6}         &   \textbf{13.2 }        &      \textbf{23.3}       &  \textbf{7.9}         &     \textbf{15.6}         \\ \hline
\end{tabular}%
\vspace{-3mm}
% \captionof{table}{\textbf{The improvement brought by using GT boxes of better quality.} We run the off-the-shelf detector on input images of 640p instead of 256p to get bounding boxes of better quality as supervision to train our model, performance are significanlly improved on all the benchmarks.}
\captionof{table}{\small \textbf{Better results from better GT boxes.} For improved bounding-box supervision, we run the off-the-shelf detector on input images of size 640p instead of 256p, leading to improved performance across the board.}
\label{tab:rebuttal_update}
}]





